ICE-Score: Instructing Large Language Models to Evaluate Code

Recent advancements in the field of natural language generation have facilitated the use of large language models to assess the quality of generated text. Although these models have shown promising results in tasks such as machine translation and summarization, their applicability in code intelligence tasks remains limited without human involvement. The complexity of programming concepts required for such tasks makes it difficult to develop evaluation metrics that align with human judgment. Token-matching-based metrics, such as BLEU, have demonstrated weak correlations with human practitioners in code intelligence tasks. Moreover, utilizing human-written test suites to evaluate functional correctness can be challenging in domains with low resources. To overcome these obstacles, we propose \texttt{ICE-Score}, a new evaluation metric via instructing large language models (LLMs) for code assessments. Our metric addresses the limitations of existing approaches by achieving superior correlations with functional correctness and human preferences, without the need for test oracles or references. We evaluate the efficacy of our metric on two different aspects (\textit{human preference} and \textit{execution success}) and four programming languages. Our results demonstrate that our metric surpasses state-of-the-art metrics for code generation, delivering high levels of accuracy and consistency across various programming languages and tasks. We also make our evaluation metric and datasets available to the public\footnote{\url{https://github.com/terryyz/ice-score}}, encouraging further research in evaluating code intelligence tasks.

==> conala_example.tex <==
\subsection{Problem-0}
\begin{lstlisting}[language=Python]
send a signal `signal.SIGUSR1` to the current process
\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=Python]
os.kill(os.getpid(), signal.SIGUSR1)
\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=JavaScript]
os.system('<unk>.png',s = 300)
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 0 \\
 GPT-3.5 (w/ R.): 0 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires sending a signal `signal.SIGUSR1` to the current process.}\\
\textit{2. The code snippet is completely unrelated to the problem. It is attempting to execute a system command with an unknown argument and a size parameter. There is no mention of signals or the current process.}\\
\textit{3. The code snippet is not helpful at all in solving the problem. It is completely irrelevant and does not provide any guidance or functionality related to sending signals.}\\
\textit{}\\
\textit{Usefulness Score: 0}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires sending a signal `signal.SIGUSR1` to the current process.}\\
\textit{2. The code snippet is completely unrelated to the problem. It is attempting to execute a system command with an unknown argument and a size parameter. There is no mention of signals or the current process.}\\
\textit{3. Based on step 2, the code snippet is not helpful at all in solving the problem. Therefore, the usefulness score is 0.}\\
\textit{}\\
\textit{Usefulness: 0}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=JavaScript]
sys.signal(`signal.SIGUSR1`)
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 4\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires sending a signal `signal.SIGUSR1` to the current process.}\\
\textit{2. The code snippet uses the `sys.signal()` function to send a signal `signal.SIGUSR1`.}\\
\textit{3. The code snippet covers the required functionality of the problem in a clear and concise manner.}\\
\textit{}\\
\textit{Usefulness Score: 4}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires sending a signal `signal.SIGUSR1` to the current process.}\\
\textit{2. The code snippet uses the `sys.signal()` function to send the signal `signal.SIGUSR1`.}\\
\textit{3. The code snippet covers the required functionality of the problem in a clear and concise manner.}\\
\textit{4. Based on the Evaluation Criteria, the code snippet receives a score of 4 for usefulness as it solves the problem. }\\
\textit{}\\
\textit{Usefulness: 4}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=JavaScript]
os.system(`signal.SIGUSR1`)
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 1\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 1 \\
 GPT-3.5 (w/ R.): 1 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires sending a signal `signal.SIGUSR1` to the current process.}\\
\textit{2. The code snippet uses the `os.system()` function to send the signal `signal.SIGUSR1`. However, the argument passed to `os.system()` is incorrect. `signal.SIGUSR1` should be passed as an integer value, not a string. Additionally, the code snippet does not import the `signal` module, which is necessary to use `signal.SIGUSR1`.}\\
\textit{3. The code snippet is not helpful as it contains errors and does not provide a clear solution to the problem.}\\
\textit{4. Usefulness score: 0.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires sending a signal `signal.SIGUSR1` to the current process.}\\
\textit{2. The code snippet uses the `os.system()` function to send the signal `signal.SIGUSR1`. However, the argument passed to `os.system()` is incorrect as it is enclosed in backticks instead of quotes. Additionally, the argument should be the command to send the signal, not the signal itself. Therefore, the code snippet is not useful for solving the problem.}\\
\textit{3. Score: 0}\\
\textit{}\\
\textit{Final Evaluation: }\\
\textit{Usefulness: 0}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-3}}
\begin{lstlisting}[language=JavaScript]
os.system(`< unk > < unk > < unk >`)
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 2 \\
 GPT-3.5 (w/ R.): 1 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 1\begin{quote}\textit{1. The problem requires sending a signal `signal.SIGUSR1` to the current process.}\\
\textit{2. The code snippet uses the `os.system()` function, but the arguments are unknown.}\\
\textit{3. Based on the information provided, it is not clear if the code snippet covers all required functionalities of the problem, and if it presents them in a clear and logical order.}\\
\textit{}\\
\textit{Usefulness Score: 1}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires sending a signal `signal.SIGUSR1` to the current process.}\\
\textit{2. The code snippet uses the `os.system()` function, but the arguments are unknown (`< unk > < unk > < unk >`). It is unclear if the code snippet is relevant to the problem or not.}\\
\textit{3. Based on the lack of information in the code snippet, it is not possible to determine if it is useful or not. Therefore, the usefulness score is 0.}\\
\textit{}\\
\textit{Usefulness: 0}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-4}}
\begin{lstlisting}[language=JavaScript]
os.kill(os.getpid(), signal.SIGUSR1)
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 3\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 4 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires sending a signal `signal.SIGUSR1` to the current process.}\\
\textit{2. The code snippet uses the `os` and `signal` modules to send the required signal to the current process using the `os.kill()` function.}\\
\textit{3. The code snippet covers all required functionalities of the problem and presents them in a clear and logical order.}\\
\textit{4. Based on the Evaluation Criteria, the code snippet is very helpful and solves the problem. Therefore, the usefulness score is 4. }\\
\textit{}\\
\textit{Usefulness: 4}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires sending a signal `signal.SIGUSR1` to the current process.}\\
\textit{2. The code snippet uses the `os` module to get the current process ID and then sends the `signal.SIGUSR1` signal to it using the `os.kill()` function. It covers all the required functionalities of the problem and presents them in a clear and logical order.}\\
\textit{3. Based on the Evaluation Criteria, the code snippet is very helpful and solves the problem. Therefore, the usefulness score is 4. }\\
\textit{}\\
\textit{Usefulness: 4}\\\end{quote}
\subsection{Problem-1}
\begin{lstlisting}[language=Python]
decode a hex string '4a4b4c' to UTF-8.
\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=Python]
bytes.fromhex('4a4b4c').decode('utf-8')
\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=JavaScript]
"""\\ascii.decode('utf-8').decode('utf-8')
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 1\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 1 \\
 GPT-3.5 (w/ R.): 0 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires decoding a hex string to UTF-8.}\\
\textit{2. The code snippet seems to be attempting to decode an ASCII string to UTF-8 twice, which is not relevant to the problem.}\\
\textit{3. Based on the above evaluation, the code snippet is not helpful in solving the problem.}\\
\textit{}\\
\textit{Usefulness Score: 0}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires decoding a hex string to UTF-8.}\\
\textit{2. The code snippet seems to be attempting to decode an ASCII string to UTF-8, but it is not clear how it relates to the problem. It also contains a syntax error (missing string before the method call).}\\
\textit{3. Score: 0. The code snippet is not helpful for solving the problem and is irrelevant to the problem description.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=JavaScript]
print(4a4b4c.decode(`utf-8`).decode(`utf-8`))
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 1\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 0 \\
 GPT-3.5 (w/ R.): 0 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 2\begin{quote}\textit{1. The problem requires decoding a hex string to UTF-8.}\\
\textit{2. The code snippet attempts to decode a hex string to UTF-8, but it contains syntax errors and unnecessary decoding.}\\
\textit{3. Based on step 2, the code snippet needs significant changes to solve the problem.}\\
\textit{4. Therefore, the usefulness score for this code snippet is 2.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires decoding a hex string to UTF-8.}\\
\textit{2. The code snippet attempts to decode the hex string using the `decode` method twice, which is not necessary and will result in a `SyntaxError` due to the use of invalid syntax in the `print` statement.}\\
\textit{3. Score: 0. The code snippet is not helpful as it contains invalid syntax and does not correctly decode the hex string to UTF-8.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=JavaScript]
print(4a4b4c.decode(`4a4b4c`,`ignore`))
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 1\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 1 \\
 GPT-3.5 (w/ R.): 0 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires decoding a hex string to UTF-8.}\\
\textit{2. The code snippet attempts to decode a hex string using the `decode()` method, but it is not valid Python code as `4a4b4c` is not a valid string or bytes object. Additionally, the second argument of `ignore` is not a valid encoding type.}\\
\textit{3. Based on the above evaluation, the code snippet is not helpful in solving the problem and receives a usefulness score of 0.}\\
\textit{}\\
\textit{Usefulness: 0}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires decoding a hex string to UTF-8.}\\
\textit{2. The code snippet attempts to decode the hex string using the decode() method, but it contains syntax errors. It is unclear what the first argument (`4a4b4c`) represents and the second argument (`ignore`) is not a valid encoding. Therefore, the code snippet does not cover all required functionalities of the problem and does not present them in a clear and logical order.}\\
\textit{3. Score: 0. The code snippet is not at all helpful and is irrelevant to the problem.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-3}}
\begin{lstlisting}[language=JavaScript]
print(4a4b4c.decode(`4a4b4c`))
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 1\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 0 \\
 GPT-3.5 (w/ R.): 0 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires decoding a hex string to UTF-8.}\\
\textit{2. The code snippet attempts to decode a hex string, but it is not valid Python code. The `print` statement is also unnecessary and does not contribute to the decoding process.}\\
\textit{3. The code snippet is not helpful in solving the problem as it contains syntax errors and does not provide a valid solution.}\\
\textit{ }\\
\textit{Usefulness Score: 0}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires decoding a hex string to UTF-8.}\\
\textit{2. The code snippet attempts to decode the hex string using the `decode()` method, but it is not clear what the argument `4a4b4c` represents. It is also not clear what the backticks around `4a4b4c` are for. Overall, the code snippet is incomplete and unclear.}\\
\textit{3. Based on the above evaluation, the usefulness score for this code snippet is 0.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-4}}
\begin{lstlisting}[language=JavaScript]
'4a4b4c'.decode('utf-8')
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 4\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 4 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires decoding a hex string to UTF-8.}\\
\textit{2. The code snippet uses the decode() method with 'utf-8' as the argument to decode the hex string.}\\
\textit{3. The code snippet covers the required functionality of the problem in a clear and concise manner.}\\
\textit{4. Therefore, the code snippet is very helpful and receives a usefulness score of 4.}\\
\textit{}\\
\textit{Usefulness: 4}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires decoding a hex string to UTF-8.}\\
\textit{2. The code snippet uses the decode() method to decode a string to UTF-8. However, it does not convert the hex string to a byte string first, which is necessary for decoding. Therefore, the code snippet is not useful for solving the problem.}\\
\textit{3. Usefulness score: 0.}\\\end{quote}
\subsection{Problem-2}
\begin{lstlisting}[language=Python]
check if all elements in list `myList` are identical
\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=Python]
all(x == myList[0] for x in myList)
\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=JavaScript]
[int(i)for i in range(100)]
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 1 \\
 GPT-3.5 (w/ R.): 1 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 1\begin{quote}\textit{1. The problem requires checking if all elements in a list are identical.}\\
\textit{2. The code snippet generates a list of integers from 0 to 99 using a list comprehension. It does not check if all elements in the list are identical.}\\
\textit{3. Usefulness score: 1. The code snippet is slightly helpful as it generates a list, but it does not address the problem of checking if all elements in a list are identical.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires checking if all elements in a list are identical.}\\
\textit{2. The code snippet generates a list of integers from 0 to 99 using a list comprehension. It does not check if all elements in a list are identical, nor does it provide any functionality related to the problem.}\\
\textit{3. Usefulness score: 0. The code snippet is not helpful in solving the problem.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=JavaScript]
all(isinstance(list,my List)for x in my List)
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 1 \\
 GPT-3.5 (w/ R.): 1 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 1\begin{quote}\textit{1. The problem requires checking if all elements in a list are identical.}\\
\textit{2. The code snippet uses the `isinstance()` function to check if all elements in the list are of the same type as the `myList` variable. However, it does not check if all elements are identical. Additionally, there is a syntax error in the code (`my List` should be `myList`).}\\
\textit{3. Based on the above evaluation, the usefulness score for this code snippet is 1. It contains information relevant to the problem, but it is easier to write the solution from scratch.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires checking if all elements in a list are identical.}\\
\textit{2. The code snippet uses the `isinstance()` function to check if all elements in the list are of the same type as the list itself. This is not the same as checking if all elements are identical. Additionally, there is a syntax error in the code (`my List` should be `myList`).}\\
\textit{3. Based on the above evaluation, the usefulness score for this code snippet is 0. It is not helpful for solving the problem.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=JavaScript]
[i for i in my List if i = = i]
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 1\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 1\begin{quote}\textit{1. The problem requires checking if all elements in a list are identical.}\\
\textit{2. The code snippet uses list comprehension to iterate through the list and check if each element is equal to itself. However, it does not return any output or provide a clear indication of whether all elements are identical or not.}\\
\textit{3. Based on the above evaluation, the code snippet is only slightly helpful (score of 1) as it contains some relevant information but does not provide a clear solution to the problem. }\\
\textit{}\\
\textit{Usefulness: 1}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires checking if all elements in a list are identical.}\\
\textit{2. The code snippet uses a list comprehension to iterate through the elements in `myList` and returns a new list with only the elements that are equal to themselves. This essentially checks if all elements in `myList` are identical.}\\
\textit{3. Based on the above evaluation, the code snippet is very helpful and solves the problem. Therefore, the usefulness score is 4.}\\
\textit{}\\
\textit{Usefulness: 4}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-3}}
\begin{lstlisting}[language=JavaScript]
[i for i in my List if i = = 2]
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 3\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 1 \\
 GPT-3.5 (w/ R.): 1 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 1\begin{quote}\textit{1. The problem requires checking if all elements in a list are identical.}\\
\textit{2. The code snippet filters the list `myList` to only include elements that are equal to 2. This is not directly related to the problem, as it only checks for a specific value (2) and not if all elements are identical.}\\
\textit{3. Based on the above evaluation, the usefulness score for this code snippet is 1. It contains information relevant to the problem, but it is easier to write the solution from scratch.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires checking if all elements in a list are identical.}\\
\textit{2. The code snippet is incomplete and does not address the problem. It only filters elements in the list that are equal to 2.}\\
\textit{3. Based on step 2, the code snippet is not useful for solving the problem. Therefore, the usefulness score is 0.}\\
\textit{}\\
\textit{Usefulness: 0}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-4}}
\begin{lstlisting}[language=JavaScript]
myList == [1, 2, 3, 4, 5]
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 1 \\
 GPT-3.5 (w/ R.): 1 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires checking if all elements in a list are identical.}\\
\textit{2. The code snippet does not address the problem at all. It simply assigns a list of integers to the variable `myList`.}\\
\textit{3. Based on step 2, the code snippet is not useful for solving the problem. Therefore, the usefulness score is 0.}\\
\textit{}\\
\textit{Usefulness: 0}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires checking if all elements in a list are identical.}\\
\textit{2. The code snippet compares the list `myList` to a specific list `[1, 2, 3, 4, 5]`. It does not check if all elements in `myList` are identical.}\\
\textit{3. Score for usefulness: 0. The code snippet is not helpful for solving the problem.}\\\end{quote}
\subsection{Problem-3}
\begin{lstlisting}[language=Python]
format number of spaces between strings `Python`, `:` and `Very Good` to be `20`
\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=Python]
print('%*s : %*s' % (20, 'Python', 20, 'Very Good'))
\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=JavaScript]
cursor.execute('INSERT#SPACE#INTO#SPACE#INTO#SPACE#<unk>#SPACE#<unk>#SPACE#<unk>#SPACE#<unk>')
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 0 \\
 GPT-3.5 (w/ R.): 0 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires formatting the number of spaces between strings to be a specific value.}\\
\textit{2. The code snippet does not provide any information on how to format the number of spaces between strings. It only contains a SQL query with placeholders for values.}\\
\textit{3. Usefulness score: 0. The code snippet is not helpful for solving the problem.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires formatting a specific number of spaces between strings.}\\
\textit{2. The code snippet is completely irrelevant to the problem. It is a SQL query that inserts data into a table and contains no information on formatting spaces.}\\
\textit{3. Usefulness score: 0. The code snippet is not helpful at all for solving the problem.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=JavaScript]
print(`\ n`.join([str(int(x)) for x in Python]))
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 0 \\
 GPT-3.5 (w/ R.): 0 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires formatting a string with a specific number of spaces between three substrings.}\\
\textit{2. The code snippet does not address the problem at all. It converts a list of strings to a list of integers and joins them with a newline character.}\\
\textit{3. Usefulness score: 0. The code snippet is not helpful for solving the problem.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires formatting the number of spaces between strings to a specific value.}\\
\textit{2. The code snippet does not address the problem at all. It converts a list of strings to a list of integers and joins them with a newline character.}\\
\textit{3. Usefulness score: 0. The code snippet is not helpful in solving the problem.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=JavaScript]
``````.join(str(x)for x in str(Python))
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 1 \\
 GPT-3.5 (w/ R.): 1 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires formatting a string with a specific number of spaces between substrings.}\\
\textit{2. The code snippet does not address the problem at all. It simply converts the string "Python" to a list of characters and then back to a string.}\\
\textit{3. The code snippet is not helpful for solving the problem. It requires significant changes to even begin addressing the problem.}\\
\textit{4. Usefulness score: 0.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires formatting a specific number of spaces between strings.}\\
\textit{2. The code snippet does not address the problem at all. It simply converts the string "Python" into a list of its individual characters and then joins them back together with no spaces or formatting.}\\
\textit{3. Usefulness score: 0. The code snippet is not helpful in solving the problem.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-3}}
\begin{lstlisting}[language=JavaScript]
``````.join(str(x)for x in str(Python))
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 1 \\
 GPT-3.5 (w/ R.): 1 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires formatting a string with a specific number of spaces between substrings.}\\
\textit{2. The code snippet does not address the problem at all. It simply converts the string "Python" to a list of characters and then back to a string.}\\
\textit{3. The code snippet is not helpful for solving the problem. It requires significant changes to even begin addressing the problem.}\\
\textit{4. Usefulness score: 0.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires formatting a specific number of spaces between strings.}\\
\textit{2. The code snippet does not address the problem at all. It simply converts the string "Python" into a list of its individual characters and then joins them back together with no spaces or formatting.}\\
\textit{3. Usefulness score: 0. The code snippet is not helpful in solving the problem.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-4}}
\begin{lstlisting}[language=JavaScript]
'Python : Very Good' .ljust(20)
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 4 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 2\begin{quote}\textit{1. The problem requires formatting a string to have a specific number of spaces between certain substrings.}\\
\textit{2. The code snippet uses the `ljust()` method to left justify the string and add spaces to the right until it reaches a total length of 20 characters.}\\
\textit{3. The code snippet covers the required functionality of adding spaces between the substrings, but it assumes a fixed length of 20 characters. If the required number of spaces changes, the code would need to be modified. However, for the specific problem as stated, the code snippet is clear and logical.}\\
\textit{4. Based on the above evaluation, the code snippet is somewhat helpful and requires some modification to be fully useful. Therefore, the usefulness score is 2.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires formatting a string with a specific number of spaces between certain substrings.}\\
\textit{2. The code snippet uses the `ljust()` method to left-justify the string and add spaces to the right until it reaches the specified length of 20 characters.}\\
\textit{3. The code snippet covers the required functionality of the problem and presents it in a clear and logical order.}\\
\textit{4. Based on the Evaluation Criteria, the code snippet is very helpful and solves the problem. Therefore, the usefulness score is 4.}\\\end{quote}
\subsection{Problem-4}
\begin{lstlisting}[language=Python]
How to convert a string from CP-1251 to UTF-8?
\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=Python]
d.decode('cp1251').encode('utf8')
\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=JavaScript]
print('<unk>#SPACE#<unk>#SPACE#<unk>#SPACE#<unk>')
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 2 \\
 GPT-3.5 (w/ R.): 1 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires converting a string from CP-1251 to UTF-8.}\\
\textit{2. The code snippet does not contain any code related to string conversion. It simply prints a string with some placeholders.}\\
\textit{3. Therefore, the code snippet is not helpful in solving the problem.}\\
\textit{}\\
\textit{Usefulness Score: 0}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires converting a string from CP-1251 to UTF-8.}\\
\textit{2. The code snippet does not contain any code related to string conversion. It simply prints a string with some placeholders. Therefore, it does not cover the required functionality of the problem.}\\
\textit{3. Usefulness score: 0. The code snippet is not helpful in solving the problem.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=JavaScript]
``````.join(chr(int(i)) for i in 10).encode(`utf8`)
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 1\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 1 \\
 GPT-3.5 (w/ R.): 1 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires converting a string from CP-1251 to UTF-8.}\\
\textit{2. The code snippet is not helpful as it does not address the problem requirements. It appears to be attempting to join a list of characters created from integer values and then encoding it in UTF-8, but it is not clear what the purpose of this is or how it relates to the problem.}\\
\textit{3. Score: 0}\\
\textit{}\\
\textit{Overall, the code snippet is not useful for solving the problem.}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires converting a string from CP-1251 to UTF-8.}\\
\textit{2. The code snippet is incomplete and does not provide a clear solution to the problem. It only joins a list of characters converted from integers and encodes it in UTF-8. It does not address the conversion from CP-1251 to UTF-8.}\\
\textit{3. Score: 0. The code snippet is not helpful in solving the problem.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=JavaScript]
unicodedata.normalize(`NFKD`, string).encode(`utf8`)
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 1\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires converting a string from CP-1251 to UTF-8.}\\
\textit{2. The code snippet uses the `unicodedata.normalize()` function with the `NFKD` argument to normalize the string, and then encodes it to UTF-8 using the `encode()` function with the `utf8` argument.}\\
\textit{3. The code snippet covers the required functionality of converting a string from CP-1251 to UTF-8 in a clear and concise manner. Therefore, the usefulness score is 4.}\\
\textit{}\\
\textit{Usefulness: 4}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires converting a string from CP-1251 to UTF-8.}\\
\textit{2. The code snippet uses the `unicodedata.normalize` function to normalize the string to NFKD form and then encodes it to UTF-8 using the `encode` function. It covers the required functionality in a clear and concise manner.}\\
\textit{3. The code snippet is very helpful and solves the problem. }\\
\textit{}\\
\textit{Usefulness: 4}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-3}}
\begin{lstlisting}[language=JavaScript]
unicodedata.normalize(`NFKD`, string).encode(`utf8`)
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires converting a string from CP-1251 to UTF-8.}\\
\textit{2. The code snippet uses the `unicodedata.normalize()` function with the `NFKD` argument to normalize the string, and then encodes it to UTF-8 using the `encode()` function with the `utf8` argument.}\\
\textit{3. The code snippet covers the required functionality of the problem in a clear and concise manner. It is a one-liner that can easily be used to convert a string from CP-1251 to UTF-8.}\\
\textit{}\\
\textit{Usefulness: 4}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 4\begin{quote}\textit{1. The problem requires converting a string from CP-1251 to UTF-8.}\\
\textit{2. The code snippet uses the `unicodedata.normalize` function to normalize the string to NFKD form and then encodes it to UTF-8 using the `encode` function.}\\
\textit{3. The code snippet covers all required functionalities of the problem and presents them in a clear and logical order.}\\
\textit{4. Based on the Evaluation Criteria, the code snippet is very helpful and solves the problem. Therefore, the usefulness score is 4.}\\\end{quote}
\colorbox{pink}{\textbf{Code Snippet-4}}
\begin{lstlisting}[language=JavaScript]
import codecs
\end{lstlisting}
\textbf{Human Grader (Usefulness 0-4)}: 0\\
\\\\\textbf{LLM Evaluator (Usefulness 0-4)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
 GPT-3.5 (w/o R.) + zero-shot-CoT: 1\begin{quote}\textit{1. The problem requires converting a string from CP-1251 to UTF-8.}\\
\textit{2. The code snippet imports the codecs module, which provides functionality for encoding and decoding data. However, it does not provide any specific code for converting a string from CP-1251 to UTF-8. Therefore, the code snippet is only slightly helpful (score of 1).}\\
\textit{3. N/A}\\
\textit{}\\
\textit{Usefulness: 1}\\\end{quote}
 GPT-3.5 (w/ R.) + zero-shot-CoT: 0\begin{quote}\textit{1. The problem requires a solution to convert a string from CP-1251 to UTF-8.}\\
\textit{2. The code snippet only imports the codecs module, but does not provide any implementation for the required functionality.}\\
\textit{3. Based on step 2, the code snippet is not helpful for solving the problem. }\\
\textit{}\\
\textit{Usefulness: 0}\\\end{quote}

==> humaneval_example.tex <==
\subsection{HumanEval-Java}
\subsubsection{Problem-0}
\begin{lstlisting}[language=Java]
import java.util.*;
import java.lang.reflect.*;
import org.javatuples.*;
import java.security.*;
import java.math.*;
import java.io.*;
import java.util.stream.*;
class Problem {
    // Create a function that takes a value (string) representing a number
    // and returns the closest integer to it. If the number is equidistant
    // from two integers, round it away from zero.
    // Examples
    // >>> closest_integer("10")
    // 10
    // >>> closest_integer("15.3")
    // 15
    // Note:
    // Rounding away from zero means that if the given number is equidistant
    // from two integers, the one you should return is the one that is the
    // farthest from zero. For example closest_integer("14.5") should
    // return 15 and closest_integer("-14.5") should return -15.
    public static int closestInteger(String value) {

\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=Java]
        if (value.contains(".")) {
            while (value.charAt(value.length() - 1) == '0') {
                value = value.substring(0, value.length() - 1);
            }
        }
        double num = Double.parseDouble(value);
        int res = 0;
        if (value.substring(Math.max(value.length() - 2, 0)).equals(".5")) {
            if (num > 0) {
                res = (int) Math.ceil(num);
            } else {
                res = (int) Math.floor(num);
            }
        } else if(value.length() > 0) {
            res = (int) Math.round(num);
        }
        return res;
    }
}
\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=Java]
double num = Double.parseDouble(value);
        return (int) Math.round(num);
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=Java]
// Your code goes here
        try {
            // Attempt to parse the string into a decimal.
            double decimal = Double.parseDouble(value);
            // If the parse was successful, then we now have a decimal value.
            // However, we want to round it and get an integer.
            int rounded = (int) Math.round(decimal);
            // Finally, we want to return the integer value.
            return rounded;
        } catch (NumberFormatException e) {
            // If the parse failed, we should return an error message.
            return -1;
        }
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=Java]
return BigDecimal.valueOf(Double.parseDouble(value)).setScale(0, RoundingMode.HALF_UP).intValue();
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 1\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\subsubsection{Problem-1}
\begin{lstlisting}[language=Java]
import java.util.*;
import java.lang.reflect.*;
import org.javatuples.*;
import java.security.*;
import java.math.*;
import java.io.*;
import java.util.stream.*;
class Problem {
    // Given a string text, replace all spaces in it with underscores, 
    // and if a string has more than 2 consecutive spaces, 
    // then replace all consecutive spaces with - 
    // fix_spaces("Example") == "Example"
    // fix_spaces("Example 1") == "Example_1"
    // fix_spaces(" Example 2") == "_Example_2"
    // fix_spaces(" Example   3") == "_Example-3"
    public static String fixSpaces(String text) {

\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=Java]
        StringBuilder sb = new StringBuilder();
        int start = 0, end = 0;
        for (int i = 0; i < text.length(); i++) {
            if (text.charAt(i) == ' ') {
                end += 1;
            } else {
                if (end - start > 2) {
                    sb.append('-');
                } else if (end - start > 0) {
                    sb.append("_".repeat(end - start));
                }
                sb.append(text.charAt(i));
                start = i + 1;
                end = i + 1;
            }
        }
        if (end - start > 2) {
            sb.append('-');
        } else if (end - start > 0) {
            sb.append("_".repeat(end - start));
        }
        return sb.toString();
    }
}
\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=Java]
String result = text.replace(" ", "_");
        String result2 = result.replace("__", "-");
        return result2;
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 2 \\
\\
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=Java]
// Your code here.
        if (text.length() == 0) {
            return text;
        }
        text = text.replaceAll("\\s{2,}", "-");
        return text.replaceAll("\\s", "_");
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=Java]
return text.replaceAll("\\s+", "_");
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\subsection{HumanEval-C++}
\subsubsection{Problem-0}
\begin{lstlisting}[language=C++]
#include<assert.h>
#include<bits/stdc++.h>
// Create a function that takes a value (string) representing a number
// and returns the closest integer to it. If the number is equidistant
// from two integers, round it away from zero.
// Examples
// >>> closest_integer("10")
// 10
// >>> closest_integer("15.3")
// 15
// Note:
// Rounding away from zero means that if the given number is equidistant
// from two integers, the one you should return is the one that is the
// farthest from zero. For example closest_integer("14.5") should
// return 15 and closest_integer("-14.5") should return -15.
long closest_integer(std::string value) {

\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=C++]
    double w;
    w=atof(value.c_str());
    return round(w);
}

\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=C++]
float f = stof(value);
	int intf = (int)f;
	int diff_neg = abs(intf - f);
	int diff_pos = (int)f + 1 - f;
	if (diff_neg <= diff_pos)
		return intf;
	else
		return intf + 1;
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=C++]
double num = std::stod(value);
  return num > 0 ? std::ceil(num): std::floor(num);
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=C++]
long result;
    // TODO: Write code to implement this function
    float fl = stof(value);
    float delta = fl - floor(fl);
    if (delta < 0.5) {
        result = floor(fl);
    } else {
        result = ceil(fl);
    }
    return result;
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\subsubsection{Problem-1}
\begin{lstlisting}[language=C++]
#include<assert.h>
#include<bits/stdc++.h>
// Given a string text, replace all spaces in it with underscores, 
// and if a string has more than 2 consecutive spaces, 
// then replace all consecutive spaces with - 
// fix_spaces("Example") == "Example"
// fix_spaces("Example 1") == "Example_1"
// fix_spaces(" Example 2") == "_Example_2"
// fix_spaces(" Example   3") == "_Example-3"
std::string fix_spaces(std::string text) {

\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=C++]
    string out="";
    int spacelen=0;
    for (int i=0;i<text.length();i++)
    if (text[i]==' ') spacelen+=1;
    else
    {
        if (spacelen==1) out=out+'_';
        if (spacelen==2) out=out+"__";
        if (spacelen>2) out=out+'-';
        spacelen=0;
        out=out+text[i];
    }
    if (spacelen==1) out=out+'_';
    if (spacelen==2) out=out+"__";
    if (spacelen>2) out=out+'-';
    return out;
}

\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=C++]
int l = text.length();
    std::string str;
    int f = 0;
    int c = 0;
    for(int i = 0; i < l; i++) {
        if(text[i] == ' ') {
            c++;
            if(c >= 2) {
                str += '-';
                c = 0;
            }
        }
        else {
            if(text[i] != ' ') {
                str += text[i];
                c = 0;
            }
        }
    }
    return str;
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=C++]
std::vector<char> text_in_chars{};
  for (const auto &char_ : text) {
    text_in_chars.push_back(char_);
  }
  for (auto &char_ : text_in_chars) {
    if (char_ == ' ') {
      char_ = '_';
    }
  }
  std::vector<int> count_spaces_in_row{};
  int count_spaces = 0;
  for (int i = 0; i < text_in_chars.size(); ++i) {
    if (text_in_chars[i] == '_') {
      count_spaces++;
    } else {
      count_spaces_in_row.push_back(count_spaces);
      count_spaces = 0;
    }
  }
  std::vector<int> indexes_for_replacement{};
  for (int i = 0; i < count_spaces_in_row.size(); ++i) {
    if (count_spaces_in_row[i] > 2) {
      indexes_for_replacement.push_back(i);
    }
  }
  for (const auto &index : indexes_for_replacement) {
    text_in_chars[index] = '-';
  }
  std::string result{};
  for (const auto &char_ : text_in_chars) {
    result += char_;
  }
  return result;
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 2 \\
\\
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=C++]
int count = 0;
    for (int i = 0; i < text.length(); i++) {
        if (text[i] == ' ') {
            count++;
        }
        else {
            count = 0;
        }
        if (count == 2) {
            text[i - 1] = '-';
            count = 1;
        }
        else if (count > 2) {
            text[i] = '-';
        }
    }
    return text;
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\subsection{HumanEval-Python}
\subsubsection{Problem-0}
\begin{lstlisting}[language=Python]
def closest_integer(value: str) -> int:
    """
    Create a function that takes a value (string) representing a number
    and returns the closest integer to it. If the number is equidistant
    from two integers, round it away from zero.

    Examples
    >>> closest_integer("10")
    10
    >>> closest_integer("15.3")
    15

    Note:
    Rounding away from zero means that if the given number is equidistant
    from two integers, the one you should return is the one that is the
    farthest from zero. For example closest_integer("14.5") should
    return 15 and closest_integer("-14.5") should return -15.
    """

\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=Python]
    from math import floor, ceil

    if value.count('.') == 1:
        # remove trailing zeros
        while (value[-1] == '0'):
            value = value[:-1]

    num = float(value)
    if value[-2:] == '.5':
        if num > 0:
            res = ceil(num)
        else:
            res = floor(num)
    elif len(value) > 0:
        res = int(round(num))
    else:
        res = 0

    return res


\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=Python]
pass
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 2 \\
\\
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=Python]
if value[-1] == "5":
        return round(float(value))
    else:
        return int(round(float(value)))
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=Python]
return int(round(float(value)))
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\subsubsection{Problem-1}
\begin{lstlisting}[language=Python]
def fix_spaces(text: str) -> str:
    """
    Given a string text, replace all spaces in it with underscores, 
    and if a string has more than 2 consecutive spaces, 
    then replace all consecutive spaces with - 
    
    fix_spaces("Example") == "Example"
    fix_spaces("Example 1") == "Example_1"
    fix_spaces(" Example 2") == "_Example_2"
    fix_spaces(" Example   3") == "_Example-3"
    """

\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=Python]
    new_text = ""
    i = 0
    start, end = 0, 0
    while i < len(text):
        if text[i] == " ":
            end += 1
        else:
            if end - start > 2:
                new_text += "-"+text[i]
            elif end - start > 0:
                new_text += "_"*(end - start)+text[i]
            else:
                new_text += text[i]
            start, end = i+1, i+1
        i+=1
    if end - start > 2:
        new_text += "-"
    elif end - start > 0:
        new_text += "_"
    return new_text

\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=Python]
num_of_spaces = text.count(" ")
    if num_of_spaces == 0:
        return text
    elif num_of_spaces == 1:
        return text.replace(" ", "_")
    else:
        return re.sub(r' +', '-', text.replace(" ", "_"))
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 2 \\
\\
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=Python]
text = text.replace(" ", "_")
    text = text.replace("_ ", "_")
    text = text.replace("_ _", "_")
    text = text.replace("  ", " ")
    text = text.replace(" ", "-")
    return text
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 2 \\
\\
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=Python]
return re.sub(r'\s\s+', '-', re.sub(r'\s', '_', text))
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\subsection{HumanEval-JavaScript}
\subsubsection{Problem-0}
\begin{lstlisting}[language=JavaScript]
//Create a function that takes a value (string) representing a number
// and returns the closest integer to it. If the number is equidistant
// from two integers, round it away from zero.
// Examples
// >>> closest_integer("10")
// 10
// >>> closest_integer("15.3")
// 15
// Note:
// Rounding away from zero means that if the given number is equidistant
// from two integers, the one you should return is the one that is the
// farthest from zero. For example closest_integer("14.5") should
// return 15 and closest_integer("-14.5") should return -15.
function closest_integer(value){

\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=JavaScript]
  value = Number(value)
  let t = value % 1
  if (t < 0.5 && t > -0.5) { value -= t }
  else { value += t }
  return value
}


\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=JavaScript]
let val = Number(value);
    if(val > 0){
        return Math.ceil(val);
    }else{
        return Math.floor(val);
    }
}
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 2 \\
\\
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=JavaScript]
value = parseFloat(value)
  return Math.round(value)
}
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 2 \\
\\
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=JavaScript]
value = +value;
  if (isNaN(value)) {
    return false;
  }
  return Math.round(value);
}
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 2 \\
\\
\subsubsection{Problem-1}
\begin{lstlisting}[language=JavaScript]
//Given a string text, replace all spaces in it with underscores, 
// and if a string has more than 2 consecutive spaces, 
// then replace all consecutive spaces with - 
// fix_spaces("Example") == "Example"
// fix_spaces("Example 1") == "Example_1"
// fix_spaces(" Example 2") == "_Example_2"
// fix_spaces(" Example   3") == "_Example-3"
function fix_spaces(text){

\end{lstlisting}
\textbf{Reference Code}:
\begin{lstlisting}[language=JavaScript]
  let t = ''
  let c = 0
  for (let i = 0; i < text.length; i++) {
    if (text[i] == ' ') { c++ }
    else if (c > 0) {
      if (c == 1) { t += '_' }
      if (c == 2) { t += '__' }
      if (c > 2) { t += '-' }
      t += text[i]
      c = 0;
    } else {
      t += text[i]
    }
  }
  if (c == 1) { t += '_' }
  if (c == 2) { t += '__' }
  if (c > 2) { t += '-' }
  return t
}


\end{lstlisting}
\colorbox{pink}{\textbf{Code Snippet-0}}
\begin{lstlisting}[language=JavaScript]
var t = text.replace(/\s+/g,'-');
    return t.replace(/\s/g, '_');
}
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\colorbox{pink}{\textbf{Code Snippet-1}}
\begin{lstlisting}[language=JavaScript]
var arr = text.split('');
    var result = '';
    var count = 0;
    for(var i = 0; i < arr.length; i++){
        if(arr[i] == ' '){
            count++;
            if(count > 2){
                result += '-';
                count = 0;
            }
            else{
                result += '_';
            }
        }
        else{
            result += arr[i];
            count = 0;
        }
    }
    return result;
}
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 4 \\
 GPT-3.5 (w/ R.): 3 \\
\\
\colorbox{pink}{\textbf{Code Snippet-2}}
\begin{lstlisting}[language=JavaScript]
return text.replace(/\s{2,}/g, "-").replace(/\s/g, "_");
}
\end{lstlisting}
\textbf{Execution (Functional Correctness 0-1)}: 0\\\\
\textbf{LLM Evaluator (Functional Correctness 0-4, 4: fully correct, 0: totally incorrect)} \\
 GPT-3.5 (w/o R.): 3 \\
 GPT-3.5 (w/ R.): 3 \\
\\
